The Rise of Health Economics: Transforming the Landscape of Economic Research

This paper explores the evolving role of health economics within economic research and publishing over the past 30 years. Historically largely a niche field, health economics has become increasingly prominent, with the share of health economics papers in top journals growing significantly. We aim to identify the factors behind this rise, examining how health economics contributes to the broader economic knowledge base and the roles distinct subfields play. Using a combination of bibliometric methods and natural language processing, we classify abstracts to define health economics. Our findings suggest that the mainstreaming of health economics is driven by innovative, high-quality research, with notable cyclicality in quality ratings that highlights the emergence and impact of distinct subfields within the discipline.

==> tables/authF1Table.tex <==
p_J>0.5     &       0.481&       0.956&       0.441\\
p_J>.327    &       0.483&       0.956&       0.442\\
p_A>0.5     &       0.708&       0.934&       0.513\\
p_A>.828    &       0.672&       0.948&       0.537\\
p_C>.997    &       0.581&       0.954&       0.501\\


==> tables/authorbased_training_data_by_journal.tex <==
\begin{tabular}{lrrrr}
\toprule
 & N training & \% training & N health & \% health \\
Journal &  &  &  &  \\
\midrule
AM ECON REV & 959 & 13.60 & 28 & 6.70 \\
ECON J & 882 & 12.51 & 52 & 12.44 \\
REV ECON STAT & 834 & 11.82 & 57 & 13.64 \\
ECONOMETRICA & 823 & 11.67 & 10 & 2.39 \\
REV ECON STUD & 651 & 9.23 & 10 & 2.39 \\
J POLIT ECON & 568 & 8.05 & 20 & 4.78 \\
J EUR ECON ASSOC & 548 & 7.77 & 16 & 3.83 \\
Q J ECON & 536 & 7.60 & 18 & 4.31 \\
J HUM RESOUR & 420 & 5.95 & 109 & 26.08 \\
RAND J ECON & 309 & 4.38 & 32 & 7.66 \\
AM ECON J-APPL ECON & 267 & 3.79 & 32 & 7.66 \\
AM ECON J-ECON POLIC & 256 & 3.63 & 34 & 8.13 \\
\midrule Total & 7,053 & 100.00 & 418 & 100.00 \\
\bottomrule
\end{tabular}


==> tables/combF1Table.tex <==
\(p_J>0.500\)&       0.960&       0.969&       0.956&       0.481&       0.956&       0.441&       0.932&       0.964&       0.923\\
\(p_J>0.327\)&       0.961&       0.969&       0.956&       0.483&       0.956&       0.442&       0.933&       0.964&       0.923\\
\(p_A>0.500\)&       0.960&       0.953&       0.943&       0.708&       0.934&       0.513&       0.945&       0.946&       0.909\\
\(p_A>0.828\)&       0.943&       0.963&       0.941&       0.672&       0.948&       0.537&       0.926&       0.957&       0.912\\
\(p_C>0.498\)&       0.972&       0.967&       0.960&       0.581&       0.954&       0.501&       0.949&       0.962&       0.929\\


==> tables/cyclicality_diff_words_08_05.tex <==
\begin{tabular}{ll}
\toprule
 & p-value \\
Word &  \\
\midrule
cost & 0.00 \\
costs & 0.00 \\
analysis & 0.00 \\
used & 0.01 \\
economic & 0.01 \\
results & 0.04 \\
child & 0.00 \\
per & 0.00 \\
evidence & 0.03 \\
treatment & 0.01 \\
\bottomrule
\end{tabular}


==> tables/cyclicality_diff_words_08_10.tex <==
\begin{tabular}{ll}
\toprule
 & p-value \\
Word &  \\
\midrule
health & 0.02 \\
cost & 0.00 \\
care & 0.01 \\
analysis & 0.00 \\
used & 0.00 \\
results & 0.03 \\
reserved. & 0.00 \\
public & 0.03 \\
different & 0.01 \\
rights & 0.05 \\
\bottomrule
\end{tabular}


==> tables/cyclicality_diff_words_09_05.tex <==
\begin{tabular}{ll}
\toprule
 & p-value \\
Word &  \\
\midrule
impact & 0.01 \\
job & 0.00 \\
per & 0.00 \\
evidence & 0.02 \\
cost & 0.01 \\
study & 0.03 \\
research & 0.00 \\
increases & 0.00 \\
chronic & 0.00 \\
program & 0.00 \\
\bottomrule
\end{tabular}


==> tables/cyclicality_diff_words_09_10.tex <==
\begin{tabular}{ll}
\toprule
 & p-value \\
Word &  \\
\midrule
health & 0.04 \\
medical & 0.08 \\
study & 0.57 \\
job & 0.05 \\
waiting & 0.00 \\
hospitals & 0.00 \\
three & 0.02 \\
life & 1.00 \\
chronic & 0.68 \\
research & 0.01 \\
\bottomrule
\end{tabular}


==> tables/journF1Table.tex <==
p_J>0.5     &       0.960&       0.969&       0.956\\
p_J>.327    &       0.961&       0.969&       0.956\\
p_A>0.5     &       0.960&       0.953&       0.943\\
p_A>.828    &       0.943&       0.963&       0.941\\
p_C>.997    &       0.972&       0.967&       0.960\\


==> tables/journalbased_training_data_by_journal.tex <==
\begin{tabular}{lrrrr}
\toprule
 & N training & \% training & N health & \% health \\
Journal &  &  &  &  \\
\midrule
J ECONOMETRICS & 3,669 & 17.95 & 0 & 0.00 \\
J PUBLIC ECON & 3,191 & 15.61 & 0 & 0.00 \\
HEALTH ECON & 2,845 & 13.92 & 2,845 & 43.04 \\
J DEV ECON & 2,485 & 12.16 & 0 & 0.00 \\
J INT ECON & 2,115 & 10.35 & 0 & 0.00 \\
J HEALTH ECON & 2,038 & 9.97 & 2,038 & 30.83 \\
EUR J HEALTH ECON & 1,350 & 6.60 & 1,350 & 20.42 \\
J LABOR ECON & 970 & 4.75 & 0 & 0.00 \\
AM ECON J-MACROECON & 537 & 2.63 & 0 & 0.00 \\
THEOR ECON & 534 & 2.61 & 0 & 0.00 \\
J ECON GROWTH & 329 & 1.61 & 0 & 0.00 \\
INT J HEALTH ECON MA & 199 & 0.97 & 199 & 3.01 \\
AM J HEALTH ECON & 178 & 0.87 & 178 & 2.69 \\
\midrule Total & 20,440 & 100.00 & 6,610 & 100.00 \\
\bottomrule
\end{tabular}


==> tables/performance_author.tex <==
\begin{tabular}{lrrrr}
\toprule
 & Precision & Recall & F1-score & N \\
\midrule
Health economics & 0.42 & 0.59 & 0.49 & 59 \\
Other fields & 0.98 & 0.96 & 0.97 & 1,317 \\
\midrule
Average & 0.70 & 0.78 & 0.73 & 1,376 \\
Weighted Average & 0.96 & 0.95 & 0.95 & 1,376 \\
\bottomrule
\end{tabular}


==> tables/performance_journal.tex <==
\begin{tabular}{lrrrr}
\toprule
 & Precision & Recall & F1-score & N \\
\midrule
Health economics & 0.91 & 0.98 & 0.95 & 669 \\
Other fields & 0.99 & 0.95 & 0.97 & 1,286 \\
\midrule
Average & 0.95 & 0.97 & 0.96 & 1,955 \\
Weighted Average & 0.96 & 0.96 & 0.96 & 1,955 \\
\bottomrule
\end{tabular}


==> tables/predictions_by_journal.tex <==
\begin{tabular}{lrrrr}
\toprule
 & N sample & N journal & N author & N ROC \\
Journal &  &  &  &  \\
\midrule
J ECONOMETRICS & 3,669 & 109 & 102 & 110 \\
J PUBLIC ECON & 3,191 & 320 & 443 & 342 \\
HEALTH ECON & 2,845 & 2,719 & 2,704 & 2,749 \\
J DEV ECON & 2,485 & 147 & 182 & 164 \\
ECON J & 2,467 & 117 & 230 & 137 \\
AM ECON REV & 2,319 & 156 & 222 & 168 \\
REV ECON STAT & 2,143 & 182 & 296 & 207 \\
J INT ECON & 2,115 & 7 & 18 & 7 \\
J HEALTH ECON & 2,038 & 1,930 & 1,967 & 1,974 \\
ECONOMETRICA & 1,688 & 40 & 42 & 42 \\
REV ECON STUD & 1,562 & 58 & 72 & 63 \\
J POLIT ECON & 1,410 & 80 & 138 & 90 \\
EUR J HEALTH ECON & 1,350 & 1,328 & 1,306 & 1,332 \\
J EUR ECON ASSOC & 1,258 & 71 & 100 & 79 \\
Q J ECON & 1,239 & 104 & 150 & 111 \\
RAND J ECON & 1,166 & 89 & 140 & 93 \\
J HUM RESOUR & 1,125 & 250 & 440 & 294 \\
J LABOR ECON & 970 & 35 & 166 & 51 \\
AM ECON J-ECON POLIC & 672 & 130 & 167 & 137 \\
AM ECON J-APPL ECON & 627 & 118 & 185 & 134 \\
AM ECON J-MACROECON & 537 & 3 & 10 & 4 \\
THEOR ECON & 534 & 7 & 6 & 7 \\
J ECON GROWTH & 329 & 19 & 16 & 19 \\
INT J HEALTH ECON MA & 199 & 198 & 193 & 198 \\
AM J HEALTH ECON & 178 & 170 & 174 & 174 \\
\midrule Total & 38,116 & 8,387 & 9,469 & 8,686 \\
\bottomrule
\end{tabular}


==> tables/ranking_rel_general.tex <==
\begin{tabular}{lp{5cm}p{5cm}p{5cm}p{5cm}}
\toprule
 & Novelty & Impact & Quality (ratio) & Quality (difference) \\
Ranking &  &  &  &  \\
\midrule
1 & Graham, C; Higuera, L; Lora, E (2011): WHICH HEALTH CONDITIONS CAUSE THE MOST UNHAPPINESS?, HEALTH ECON & Mussa, R (2016): Exit from catastrophic health payments, INT J HEALTH ECON MA & Lundborg, P; Andersson, H (2008): Gender, risk perceptions, and smoking behavior, J HEALTH ECON & Lundborg, P; Andersson, H (2008): Gender, risk perceptions, and smoking behavior, J HEALTH ECON \\
2 & Duncan, B; Mansour, H; Rees, DI (2017): It's Just a Game The Super Bowl and Low Birth Weight, J HUM RESOUR & Abasolo, I; Tsuchiya, A (2004): Exploring social welfare functions and violation of monotonicity, J HEALTH ECON & Park, C; Kang, C (2008): Does education induce healthy lifestyle?, J HEALTH ECON & Park, C; Kang, C (2008): Does education induce healthy lifestyle?, J HEALTH ECON \\
3 & Anderson, PM; Butcher, KF (2006): Reading, writing, and refreshments - Are school finances contributing to children's obesity?, J HUM RESOUR & Chib, S; Jacobi, L (2008): Analysis of treatment response data from eligibility designs, J ECONOMETRICS & Currie, J; Decker, S; Lin, WC (2008): Has public health insurance for older children reduced disparities in access to care and health outcomes?, J HEALTH ECON & Currie, J; Decker, S; Lin, WC (2008): Has public health insurance for older children reduced disparities in access to care and health outcomes?, J HEALTH ECON \\
4 & Schanzenbach, DW (2009): Do School Lunches Contribute to Childhood Obesity?, J HUM RESOUR & Lorenz, N (2017): Using Quantile and Asymmetric Least Squares Regression for Optimal Risk Adjustment, HEALTH ECON & Carlsen, F; Grytten, J; Kjelvik, J; Skau, I (2007): Better primary physician services lead to fewer hospital admissions, EUR J HEALTH ECON & Carlsen, F; Grytten, J; Kjelvik, J; Skau, I (2007): Better primary physician services lead to fewer hospital admissions, EUR J HEALTH ECON \\
5 & Hamilton, BH; Hamilton, VH; Mayo, NE (1996): What are the costs of queuing for hip fracture surgery in Canada?, J HEALTH ECON & Lanscar, E; Savage, E (2004): Deriving welfare measures from discrete choice experiments, HEALTH ECON & Mossialos, E (1997): Citizens' views on health care systems in the 15 member states of the European Union, HEALTH ECON & vanDoorslaer, E; Wagstaff, A; Bleichrodt, H; Calonge, S; Gerdtham, UG; Gerfin, M; Geurts, J; Gross, L; Hakkinen, U; Leu, RE; ODonnell, O; Propper, C; Puffer, F; Rodriguez, M; Sundberg, G; Winkelhake, O (1997): Income-related inequalities in health, J HEALTH ECON \\
6 & Francesconi, M; Jenkins, SP; Siedler, T (2010): THE EFFECT OF LONE MOTHERHOOD ON THE SMOKING BEHAVIOR OF YOUNG ADULTS, HEALTH ECON & Attema, AE; Krol, M; van Exel, J; Brouwer, WBF (2018): New findings from the time trade-off for income approach to elicit willingness to pay for a quality adjusted life year, EUR J HEALTH ECON & Sabia, JJ; Rees, DI (2008): The effect of adolescent virginity status on psychological well-being, J HEALTH ECON & Pagán, JA; Puig, A; Soldo, BJ (2007): Health insurance coverage and the use of preventive services by Mexican adults, HEALTH ECON \\
7 & Chiu, WH (1997): Health insurance and the welfare of health care consumers, J PUBLIC ECON & Herwartz, H; Theilen, B (2010): THE DETERMINANTS OF HEALTH-CARE EXPENDITURE, HEALTH ECON & Puig-Junoy, J; Casas, A; Font-Planells, J; Escarrabill, J; Hernández, C; Alonso, J; Farrero, E; Vilagut, G; Roca, J (2007): The impact of home hospitalization on healthcare costs of exacerbations in COPD patients, EUR J HEALTH ECON & Puig-Junoy, J; Casas, A; Font-Planells, J; Escarrabill, J; Hernández, C; Alonso, J; Farrero, E; Vilagut, G; Roca, J (2007): The impact of home hospitalization on healthcare costs of exacerbations in COPD patients, EUR J HEALTH ECON \\
8 & Cawley, J; Maclean, JC (2012): UNFIT FOR SERVICE, HEALTH ECON & Manca, A; Rice, N; Sculpher, MJ; Briggs, AH (2005): Assessing generalisability by location in trial-based cost-effectiveness analysis, HEALTH ECON & vanDoorslaer, E; Wagstaff, A; Bleichrodt, H; Calonge, S; Gerdtham, UG; Gerfin, M; Geurts, J; Gross, L; Hakkinen, U; Leu, RE; ODonnell, O; Propper, C; Puffer, F; Rodriguez, M; Sundberg, G; Winkelhake, O (1997): Income-related inequalities in health, J HEALTH ECON & Mossialos, E (1997): Citizens' views on health care systems in the 15 member states of the European Union, HEALTH ECON \\
9 & Grytten, J; Rongen, G; Asmyhr, O (1996): Subsidized dental care for young men, HEALTH ECON & Anthun, KS; Bjorngaard, JH; Magnussen, J (2017): Economic incentives and diagnostic coding in a public health care system, INT J HEALTH ECON MA & Pagán, JA; Puig, A; Soldo, BJ (2007): Health insurance coverage and the use of preventive services by Mexican adults, HEALTH ECON & Bjegovic, V; Terzic, Z; Marinkovic, J; Lalic, N; Sipetic, S; Laaser, U (2007): The burden of type 2 diabetes in Serbia and the cost-effectiveness of its management, EUR J HEALTH ECON \\
10 & Courtemanche, C; Marton, J; Yelowitz, A (2016): WHO GAINED INSURANCE COVERAGE IN 2014, THE FIRST YEAR OF FULL ACA IMPLEMENTATION?, HEALTH ECON & Deb, P; Trivedi, PK; Zimmer, DM (2014): COST-OFFSETS OF PRESCRIPTION DRUG EXPENDITURES, HEALTH ECON & Cawley, J; Meyerhoefer, C; Newhousec, D (2007): The impact of state physical education requirements on youth physical activity and overweight, HEALTH ECON & Waters, HR; Hatt, LE; Black, RE (2008): The role of private providers in treating child diarrhoea in Latin America, HEALTH ECON \\
\bottomrule
\end{tabular}


==> tables/ranking_rel_health.tex <==
\begin{tabular}{lp{5cm}p{5cm}p{5cm}p{5cm}}
\toprule
 & Novelty & Impact & Quality (ratio) & Quality (difference) \\
Ranking &  &  &  &  \\
\midrule
1 & Kaushal, N (2005): New immigrants' location choices, J LABOR ECON & Herwartz, H; Theilen, B (2010): THE DETERMINANTS OF HEALTH-CARE EXPENDITURE, HEALTH ECON & Sonnad, SS; Foreman, SE (1997): An incentive approach to physician implementation of medical practice guidelines, HEALTH ECON & Sonnad, SS; Foreman, SE (1997): An incentive approach to physician implementation of medical practice guidelines, HEALTH ECON \\
2 & Duncan, B; Mansour, H; Rees, DI (2017): It's Just a Game The Super Bowl and Low Birth Weight, J HUM RESOUR & Blomqvist, Å (2002): QALYs, standard gambles, and the expected budget constraint, J HEALTH ECON & Almond, D; Edlund, L; Palme, M (2009): CHERNOBYL'S SUBCLINICAL LEGACY, Q J ECON & Almond, D; Edlund, L; Palme, M (2009): CHERNOBYL'S SUBCLINICAL LEGACY, Q J ECON \\
3 & Johnson, DKN; Popp, D (2003): Forced out of the closet, RAND J ECON & Anthun, KS; Bjorngaard, JH; Magnussen, J (2017): Economic incentives and diagnostic coding in a public health care system, INT J HEALTH ECON MA & Carpenter, C; Dobkin, C (2009): The Effect of Alcohol Consumption on Mortality, AM ECON J-APPL ECON & Folmer, K; Stevens, J; VanTulder, F; Westerhout, E (1997): Towards an economic model of the Dutch health care sector, HEALTH ECON \\
4 & Hill, AJ (2015): The Girl Next Door, AM ECON J-APPL ECON & Liu, XP; Nestic, D; Vukina, T (2012): ESTIMATING ADVERSE SELECTION AND MORAL HAZARD EFFECTS WITH HOSPITAL INVOICES DATA IN A GOVERNMENT-CONTROLLED HEALTHCARE SYSTEM, HEALTH ECON & Folmer, K; Stevens, J; VanTulder, F; Westerhout, E (1997): Towards an economic model of the Dutch health care sector, HEALTH ECON & Carpenter, C; Dobkin, C (2009): The Effect of Alcohol Consumption on Mortality, AM ECON J-APPL ECON \\
5 & Francesconi, M; Jenkins, SP; Siedler, T (2010): THE EFFECT OF LONE MOTHERHOOD ON THE SMOKING BEHAVIOR OF YOUNG ADULTS, HEALTH ECON & Akin, JS; Guilkey, DK; Hutchinson, PL; McIntosh, MT (1998): Price elasticities of demand for curative health care with control for sample selectivity on endogenous illness, HEALTH ECON & Case, A; Lubotsky, D; Paxson, C (2002): Economic status and health in childhood, AM ECON REV & Wagstaff, A; van Doorslaer, E (1997): Progressivity, horizontal equity and reranking in health care finance, J HEALTH ECON \\
6 & Cooper, B; Gehrsitz, M; McIntyre, SG (2020): Drink, death, and driving, HEALTH ECON & Ament, A; Baltussen, R (1997): The interpretation of results of economic evaluation, HEALTH ECON & Wagstaff, A; van Doorslaer, E (1997): Progressivity, horizontal equity and reranking in health care finance, J HEALTH ECON & Case, A; Lubotsky, D; Paxson, C (2002): Economic status and health in childhood, AM ECON REV \\
7 & DeLeire, T (2000): The wage and employment effects of the Americans with Disabilities Act, J HUM RESOUR & Mitra, N; Indurkhya, A (2005): Propensity score approach to estimating the cost - effectiveness of medical therapies from observational data, HEALTH ECON & Jayachandran, S (2009): Air Quality and Early-Life Mortality Evidence from Indonesia's Wildfires, J HUM RESOUR & Langkilde, LK; Sogaard, J (1997): The adjustment of cost measurement to account for learning, HEALTH ECON \\
8 & Anderson, PM; Butcher, KF (2006): Reading, writing, and refreshments - Are school finances contributing to children's obesity?, J HUM RESOUR & Herwartz, H; Theilen, B (2003): The determinants of health care expenditure, HEALTH ECON & Blau, DM (1999): The effect of child care characteristics on child development, J HUM RESOUR & Olsen, JA (1997): Theories of justice and their implications for priority setting in health care, J HEALTH ECON \\
9 & Joyce, T (2009): A SIMPLE TEST OF ABORTION AND CRIME, REV ECON STAT & Martin, S; Rice, N; Smith, PC (2008): Does health care spending improve health outcomes? Evidence-from English programme budgeting data, J HEALTH ECON & Beegle, K; Dehejia, R; Gatti, R (2009): Why Should We Care About Child Labor? The Education, Labor Market, and Health Consequences of Child Labor, J HUM RESOUR & Jayachandran, S (2009): Air Quality and Early-Life Mortality Evidence from Indonesia's Wildfires, J HUM RESOUR \\
10 & Currie, J; Schwandt, H (2016): The 9/11 Dust Cloud and Pregnancy Outcomes A Reconsideration, J HUM RESOUR & d'Uva, TB (2006): Latent class models for utilisation of health care, HEALTH ECON & Langkilde, LK; Sogaard, J (1997): The adjustment of cost measurement to account for learning, HEALTH ECON & Beegle, K; Dehejia, R; Gatti, R (2009): Why Should We Care About Child Labor? The Education, Labor Market, and Health Consequences of Child Labor, J HUM RESOUR \\
\bottomrule
\end{tabular}


==> tables/tab_ols_rel_cit.tex <==
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                &No. Citations&No. Citations&No. Citations&No. Citations&No. Citations&No. Citations&No. Citations&No. Citations\\
\hline
Novelty         &    0.149&         &         &         &    2.345&    4.563&    2.345&    2.345\\
                &  [0.019]&         &         &         &  [0.425]&  [8.949]&  [0.425]&  [0.425]\\
Impact          &         &   -0.138&         &         &    2.200&    4.386&    2.200&    2.201\\
                &         &  [0.019]&         &         &  [0.426]&  [8.819]&  [0.426]&  [0.426]\\
Quality (ratio) &         &         &    0.226&         &         &   -0.191&         &         \\
                &         &         &  [0.035]&         &         &  [0.771]&         &         \\
Quality (difference)&         &         &         &    0.224&         &         &    0.000&         \\
                &         &         &         &  [0.035]&         &         &      [.]&         \\
Novelty $\times$ Impact&         &         &         &         &         &         &         &   -0.001\\
                &         &         &         &         &         &         &         &  [0.014]\\
Year FEs        &      Yes&      Yes&      Yes&      Yes&      Yes&      Yes&      Yes&      Yes\\
\hline
Observations    &     7,911&     7,911&     7,911&     7,911&     7,911&     7,911&     7,911&     7,911\\
Adjusted \(R^{2}\)&    0.004&    0.003&    0.007&    0.007&    0.011&    0.011&    0.011&    0.011\\


==> tables/tab_ols_rel_cit_residualized.tex <==
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                &No. Citations&No. Citations&No. Citations&No. Citations&No. Citations&No. Citations\\
\hline
Novelty         &    1.679&         &    2.522&   -7.241&   -8.222&    2.521\\
                &  [0.388]&         &  [0.469]&  [1.408]&  [1.498]&  [0.467]\\
Impact          &         &    0.939&    2.016&   -7.613&   -8.580&    2.013\\
                &         &  [0.403]&  [0.486]&  [1.444]&  [1.529]&  [0.474]\\
Quality (ratio) &         &         &         &    0.842&         &         \\
                &         &         &         &  [0.114]&         &         \\
Quality (difference)&         &         &         &         &    0.925&         \\
                &         &         &         &         &  [0.121]&         \\
Novelty $\times$ Impact&         &         &         &         &         &    0.598\\
                &         &         &         &         &         &  [5.380]\\
Year FEs        &      Yes&      Yes&      Yes&      Yes&      Yes&      Yes\\
\hline
Observations    &     7,911&     7,911&     7,911&     7,911&     7,911&     7,911\\
Adjusted \(R^{2}\)&    0.000&   -0.002&    0.004&    0.011&    0.011&    0.004\\


==> tables/tab_ols_rel_ref.tex <==
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                &No. References&No. References&No. References&No. References&No. References&No. References&No. References&No. References\\
\hline
Novelty         &    0.035&         &         &         &    0.195&    3.209&    0.195&    0.194\\
                &  [0.005]&         &         &         &  [0.078]&  [2.485]&  [0.078]&  [0.077]\\
Impact          &         &   -0.034&         &         &    0.160&    3.130&    0.160&    0.159\\
                &         &  [0.005]&         &         &  [0.077]&  [2.448]&  [0.077]&  [0.077]\\
Quality (ratio) &         &         &    0.023&         &         &   -0.260&         &         \\
                &         &         &  [0.007]&         &         &  [0.214]&         &         \\
Quality (difference)&         &         &         &    0.023&         &         &    0.000&         \\
                &         &         &         &  [0.007]&         &         &      [.]&         \\
Novelty $\times$ Impact&         &         &         &         &         &         &         &    0.001\\
                &         &         &         &         &         &         &         &  [0.004]\\
Year FEs        &      Yes&      Yes&      Yes&      Yes&      Yes&      Yes&      Yes&      Yes\\
\hline
Observations    &     7,910&     7,910&     7,910&     7,910&     7,910&     7,910&     7,910&     7,910\\
Adjusted \(R^{2}\)&    0.002&    0.002&   -0.002&   -0.002&    0.002&    0.003&    0.002&    0.002\\


==> tables/tab_ols_rel_ref_residualized.tex <==
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                &No. References&No. References&No. References&No. References&No. References&No. References\\
\hline
Novelty         &    0.216&         &    0.256&   -2.019&   -2.301&    0.258\\
                &  [0.083]&         &  [0.091]&  [0.374]&  [0.407]&  [0.091]\\
Impact          &         &   -0.013&    0.097&   -2.147&   -2.425&    0.107\\
                &         &  [0.084]&  [0.092]&  [0.368]&  [0.399]&  [0.092]\\
Quality (ratio) &         &         &         &    0.196&         &         \\
                &         &         &         &  [0.031]&         &         \\
Quality (difference)&         &         &         &         &    0.220&         \\
                &         &         &         &         &  [0.034]&         \\
Novelty $\times$ Impact&         &         &         &         &         &   -2.004\\
                &         &         &         &         &         &  [1.113]\\
Year FEs        &      Yes&      Yes&      Yes&      Yes&      Yes&      Yes\\
\hline
Observations    &     7,910&     7,910&     7,910&     7,910&     7,910&     7,910\\
Adjusted \(R^{2}\)&   -0.003&   -0.004&   -0.003&    0.002&    0.003&   -0.002\\

